Passive Entropy Rate Bounds the Information Required for Feedback Control

Living organisms across scales, along with many engineered devices, must control noisy systems with limited information to maintain a desired steady state. Here we ask how the performance of a feedback controller is limited by the rate at which information flows from sensors to control actions. We demonstrate that the minimum information rate required is the rate at which the passive dynamics increase the system's entropy. This general result allows us to quantify the information required to achieve a given target performance for a wide-ranging set of control problems. Next, we ask what explicit control protocol maximizes performance for a given information rate. We demonstrate that in many cases the best control strategy is to probabilistically time-reverse the uncontrolled passive dynamics. Implementing this protocol approaches or saturates our bound across a wide range of applications. We showcase these results through applications to stochastic bit control, nonlinear particle localization, microbial navigation, and experimentally realized information engines. Our findings pave the way for the study of feedback control in any settings where limited information is a key constraint, suggest principled explanations for microbial behavior, and provide new insights into fundamental questions regarding the thermodynamic value of information.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
